The Tate conjecture for K3 surfaces in odd characteristic

We show that the classical Kuga-Satake construction gives rise, away from characteristic 2, to an open immersion from the moduli of primitively polarized K3 surfaces (of any fixed degree) to a certain regular integral model for a Shimura variety of orthogonal type. This allows us to attach to every polarized K3 surface in odd characteristic an abelian variety such that divisors on the surface can be identified with certain endomorphisms of the attached abelian variety. In turn, this reduces the Tate conjecture for K3 surfaces over finitely generated fields of odd characteristic to a version of the Tate conjecture for certain endomorphisms on the attached Kuga-Satake abelian variety, which we prove. As a by-product of our methods, we also show that the moduli stack of primitively polarized K3 surfaces of degree 2d is quasi-projective and, when d is not divisible by p^2, is geometrically irreducible in characteristic p. We indicate how the same method applies to prove the Tate conjecture for co-dimension 2 cycles on cubic fourfolds.

==> tatek3.tex <==
Fix a small enough compact open $K^p\subset G(\Adele_f^p)$ such that $\mathsf{M}_{2d,K,\Int_{(p)}}$ is an algebraic space; here, $K=K_pK^p$.

\begin{prp}\label{tatek3:prp:special}
For every point $s\to\mathsf{M}_{2d,K,\Int_{(p)}}$ valued in a field $k(s)$, there is a natural inclusion of $\Int_{(p)}$-quadratic spaces
\[
  \on{AH}\bigl(\bm{V}_{s}\bigr)\into\langle\bm{\xi}_s\rangle^{\perp}\subset\Pic\bigl(\bm{X}_s\bigr)\otimes\Int_{(p)}
\]
compatible with cycle class maps.
\end{prp}

Before giving a proof, we show how this easily implies the Tate conjecture in many cases.
\begin{proof}[Proof of Theorem \ref{intro:thm:main}]
After replacing $k$ by a finite extension, we can assume that $X$ admits a quasi-polarization $\xi$ of degree $2d$, for some $d$. Then, extending $k$ again if necessary, we can assume that there is a point $s\in\mathsf{M}_{2d,K,\Int_{(p)}}(k)$ such that $\bm{X}_s=X$. The Tate conjecture for $X$ now follows from (\ref{tatek3:prp:special}) above and (\ref{ortho:thm:special}).
\end{proof}

\begin{proof}[Proof of (\ref{tatek3:prp:special})]
We observe that, for any element $f\in\on{AH}\bigl(\bm{V}_s\bigr)$, the corresponding element of $\Pic\bigl(\bm{X}_s\bigr)\otimes\Int_{(p)}$, if it exists, is uniquely determined by the requirement that its cohomological cycle classes agree with those of $f$.

Assume first that $k(s)$ is of characteristic $0$. Since $\bm{V}_s$ and $\bm{P}^2_s(1)\otimes\Int_{(p)}$ are identified as motives over $k(s)$, we have an identification:
\[
 \on{AH}\bigl(\bm{V}_{s}\bigr)=\on{AH}\bigl(\bm{P}^2_s(1)\bigr)\otimes\Int_{(p)}.
\]
This is clearly compatible with cycle classes. To conclude the proof in this case, we only have to observe that, by the Lefschetz $(1,1)$ theorem, we can naturally identify the right hand side with
\[
\langle\bm{\xi}_s\rangle^{\perp}\subset\Pic\bigl(\bm{X}_{s}\bigr)\otimes\Int_{(p)}.
\]

Now suppose that $k(s)$ has characteristic $p$. We can assume that $k(s)$ is perfect: Indeed, both $\Pic(\bm{X}_s)$ and $\on{AH}(\bm{V}_s)$ remain unaffected by a purely inseparable base change. Given $f\in\on{AH}\bigl(\bm{V}_s\bigr)$, we see from (\ref{ks:thm:kugasatakecharp}) and (\ref{ortho:prp:specialdeform}) that the relative deformation functor for $f$ over $\bigl(\mathsf{M}_{2d,K,\Int_{(p)}}\bigr)^{\wedge}_s$ is represented by a closed formal sub-scheme that has at least one component that is flat over $\Int_p$. In particular, we can find a finite extension $L/W(k(s))_{\Rat}$ and a lift $\widetilde{s}:\Spec\Reg{L}\to\mathsf{M}_{2d,K,\Int_{(p)}}$ of $s$, such that $f$ lifts to an element $\widetilde{f}\in\on{AH}\bigl(\bm{V}_{\widetilde{s}}\bigr)$. By the previous paragraph, this gives rise to a canonical element $\eta(\widetilde{f})\in\Pic\bigl(\bm{X}_{\widetilde{s}}\bigr)\otimes\Int_{(p)}$, with the same cohomological cycle classes as $\widetilde{f}$. Reducing this element back over $k(s)$ gives us the element of $\Pic\bigl(\bm{X}_s\bigr)\otimes\Int_{(p)}$ corresponding to $f$.
\end{proof}

\begin{rem}\label{tatek3:rem:arbit}
(\ref{tatek3:prp:special}) combined with the Tate conjecture shows that $\on{AH}(\bm{V}_s)=\Pic(\bm{X}_s)$, for all closed points $s$. Using this and a little more argument, one can show that $\on{AH}(\bm{V}_T)=\Pic(\bm{X}_T/T)$, for all $\on{M}_{2d,K,\Int_{(p)}}$-schemes $T$.
\end{rem}

